A Coalitional Game for Demand-Side Management in a Micro-Grid with Multiple Electricity Retailers

This paper develops a demand-side management framework for electricity networks with multiple competing retailers. The interaction among retailers is formulated as a coalitional game, yielding a family of coupled mixed-integer optimisation problems in which retail prices, consumer power demands, and the network partition are jointly optimised. To solve this problem, we propose a coalition-formation algorithm based on multi-objective optimisation principles. The algorithm seeks to identify coalition structures that balance retailer profit and consumer welfare. We prove that the proposed algorithm converges in a finite number of steps and recovers a subset of weakly Pareto-efficient solutions of the coupled optimisation problems. The framework is further extended to a risk-sharing formulation, in which the objective is defined using conditional value-at-risk. Numerical simulations on an academic example demonstrate the method's behaviour and show that the resulting equilibrium partition set contains several admissible trade-offs between the competing objectives. The results provide a tractable approach for analysing competition, coalition formation, and risk-aware pricing in multi-retailer demand-side management systems.

==> figs/colormap_def.tex <==
\pgfplotsset{
    /pgfplots/colormap={mycolormap}{
        rgb=(1.00000, 1.00000, 1.00000)
        rgb=(0.00331, 0.79669, 0.79669)
        rgb=(0.00661, 0.79339, 0.79339)
        rgb=(0.00992, 0.79008, 0.79008)
        rgb=(0.01322, 0.78678, 0.78678)
        rgb=(0.01653, 0.78347, 0.78347)
        rgb=(0.01983, 0.78017, 0.78017)
        rgb=(0.02314, 0.77686, 0.77686)
        rgb=(0.02645, 0.77355, 0.77355)
        rgb=(0.02975, 0.77025, 0.77025)
        rgb=(0.03306, 0.76694, 0.76694)
        rgb=(0.03636, 0.76364, 0.76364)
        rgb=(0.03967, 0.76033, 0.76033)
        rgb=(0.04298, 0.75702, 0.75702)
        rgb=(0.04628, 0.75372, 0.75372)
        rgb=(0.04959, 0.75041, 0.75041)
        rgb=(0.05289, 0.74711, 0.74711)
        rgb=(0.05620, 0.74380, 0.74380)
        rgb=(0.05950, 0.74050, 0.74050)
        rgb=(0.06281, 0.73719, 0.73719)
        rgb=(0.06612, 0.73388, 0.73388)
        rgb=(0.06942, 0.73058, 0.73058)
        rgb=(0.07273, 0.72727, 0.72727)
        rgb=(0.07603, 0.72397, 0.72397)
        rgb=(0.07934, 0.72066, 0.72066)
        rgb=(0.08264, 0.71736, 0.71736)
        rgb=(0.08595, 0.71405, 0.71405)
        rgb=(0.08926, 0.71074, 0.71074)
        rgb=(0.09256, 0.70744, 0.70744)
        rgb=(0.09587, 0.70413, 0.70413)
        rgb=(0.09917, 0.70083, 0.70083)
        rgb=(0.10248, 0.69752, 0.69752)
        rgb=(0.10579, 0.69421, 0.69421)
        rgb=(0.10909, 0.69091, 0.69091)
        rgb=(0.11240, 0.68760, 0.68760)
        rgb=(0.11570, 0.68430, 0.68430)
        rgb=(0.11901, 0.68099, 0.68099)
        rgb=(0.12231, 0.67769, 0.67769)
        rgb=(0.12562, 0.67438, 0.67438)
        rgb=(0.12893, 0.67107, 0.67107)
        rgb=(0.13223, 0.66777, 0.66777)
        rgb=(0.13554, 0.66446, 0.66446)
        rgb=(0.13884, 0.66116, 0.66116)
        rgb=(0.14215, 0.65785, 0.65785)
        rgb=(0.14545, 0.65455, 0.65455)
        rgb=(0.14876, 0.65124, 0.65124)
        rgb=(0.15207, 0.64793, 0.64793)
        rgb=(0.15537, 0.64463, 0.64463)
        rgb=(0.15868, 0.64132, 0.64132)
        rgb=(0.16198, 0.63802, 0.63802)
        rgb=(0.16529, 0.63471, 0.63471)
        rgb=(0.16860, 0.63140, 0.63140)
        rgb=(0.17190, 0.62810, 0.62810)
        rgb=(0.17521, 0.62479, 0.62479)
        rgb=(0.17851, 0.62149, 0.62149)
        rgb=(0.18182, 0.61818, 0.61818)
        rgb=(0.18512, 0.61488, 0.61488)
        rgb=(0.18843, 0.61157, 0.61157)
        rgb=(0.19174, 0.60826, 0.60826)
        rgb=(0.19504, 0.60496, 0.60496)
        rgb=(0.19835, 0.60165, 0.60165)
        rgb=(0.20165, 0.59835, 0.59835)
        rgb=(0.20496, 0.59504, 0.59504)
        rgb=(0.20826, 0.59174, 0.59174)
        rgb=(0.21157, 0.58843, 0.58843)
        rgb=(0.21488, 0.58512, 0.58512)
        rgb=(0.21818, 0.58182, 0.58182)
        rgb=(0.22149, 0.57851, 0.57851)
        rgb=(0.22479, 0.57521, 0.57521)
        rgb=(0.22810, 0.57190, 0.57190)
        rgb=(0.23140, 0.56860, 0.56860)
        rgb=(0.23471, 0.56529, 0.56529)
        rgb=(0.23802, 0.56198, 0.56198)
        rgb=(0.24132, 0.55868, 0.55868)
        rgb=(0.24463, 0.55537, 0.55537)
        rgb=(0.24793, 0.55207, 0.55207)
        rgb=(0.25124, 0.54876, 0.54876)
        rgb=(0.25455, 0.54545, 0.54545)
        rgb=(0.25785, 0.54215, 0.54215)
        rgb=(0.26116, 0.53884, 0.53884)
        rgb=(0.26446, 0.53554, 0.53554)
        rgb=(0.26777, 0.53223, 0.53223)
        rgb=(0.27107, 0.52893, 0.52893)
        rgb=(0.27438, 0.52562, 0.52562)
        rgb=(0.27769, 0.52231, 0.52231)
        rgb=(0.28099, 0.51901, 0.51901)
        rgb=(0.28430, 0.51570, 0.51570)
        rgb=(0.28760, 0.51240, 0.51240)
        rgb=(0.29091, 0.50909, 0.50909)
        rgb=(0.29421, 0.50579, 0.50579)
        rgb=(0.29752, 0.50248, 0.50248)
        rgb=(0.30083, 0.49917, 0.49917)
        rgb=(0.30413, 0.49587, 0.49587)
        rgb=(0.30744, 0.49256, 0.49256)
        rgb=(0.31074, 0.48926, 0.48926)
        rgb=(0.31405, 0.48595, 0.48595)
        rgb=(0.31736, 0.48264, 0.48264)
        rgb=(0.32066, 0.47934, 0.47934)
        rgb=(0.32397, 0.47603, 0.47603)
        rgb=(0.32727, 0.47273, 0.47273)
        rgb=(0.33058, 0.46942, 0.46942)
        rgb=(0.33388, 0.46612, 0.46612)
        rgb=(0.33719, 0.46281, 0.46281)
        rgb=(0.34050, 0.45950, 0.45950)
        rgb=(0.34380, 0.45620, 0.45620)
        rgb=(0.34711, 0.45289, 0.45289)
        rgb=(0.35041, 0.44959, 0.44959)
        rgb=(0.35372, 0.44628, 0.44628)
        rgb=(0.35702, 0.44298, 0.44298)
        rgb=(0.36033, 0.43967, 0.43967)
        rgb=(0.36364, 0.43636, 0.43636)
        rgb=(0.36694, 0.43306, 0.43306)
        rgb=(0.37025, 0.42975, 0.42975)
        rgb=(0.37355, 0.42645, 0.42645)
        rgb=(0.37686, 0.42314, 0.42314)
        rgb=(0.38017, 0.41983, 0.41983)
        rgb=(0.38347, 0.41653, 0.41653)
        rgb=(0.38678, 0.41322, 0.41322)
        rgb=(0.39008, 0.40992, 0.40992)
        rgb=(0.39339, 0.40661, 0.40661)
        rgb=(0.39669, 0.40331, 0.40331)
        rgb=(0.40000, 0.40000, 0.40000)
        rgb=(0.40331, 0.39669, 0.39669)
        rgb=(0.40661, 0.39339, 0.39339)
        rgb=(0.40992, 0.39008, 0.39008)
        rgb=(0.41322, 0.38678, 0.38678)
        rgb=(0.41653, 0.38347, 0.38347)
        rgb=(0.41983, 0.38017, 0.38017)
        rgb=(0.42314, 0.37686, 0.37686)
        rgb=(0.42645, 0.37355, 0.37355)
        rgb=(0.42975, 0.37025, 0.37025)
        rgb=(0.43306, 0.36694, 0.36694)
        rgb=(0.43636, 0.36364, 0.36364)
        rgb=(0.43967, 0.36033, 0.36033)
        rgb=(0.44298, 0.35702, 0.35702)
        rgb=(0.44628, 0.35372, 0.35372)
        rgb=(0.44959, 0.35041, 0.35041)
        rgb=(0.45289, 0.34711, 0.34711)
        rgb=(0.45620, 0.34380, 0.34380)
        rgb=(0.45950, 0.34050, 0.34050)
        rgb=(0.46281, 0.33719, 0.33719)
        rgb=(0.46612, 0.33388, 0.33388)
        rgb=(0.46942, 0.33058, 0.33058)
        rgb=(0.47273, 0.32727, 0.32727)
        rgb=(0.47603, 0.32397, 0.32397)
        rgb=(0.47934, 0.32066, 0.32066)
        rgb=(0.48264, 0.31736, 0.31736)
        rgb=(0.48595, 0.31405, 0.31405)
        rgb=(0.48926, 0.31074, 0.31074)
        rgb=(0.49256, 0.30744, 0.30744)
        rgb=(0.49587, 0.30413, 0.30413)
        rgb=(0.49917, 0.30083, 0.30083)
        rgb=(0.50248, 0.29752, 0.29752)
        rgb=(0.50579, 0.29421, 0.29421)
        rgb=(0.50909, 0.29091, 0.29091)
        rgb=(0.51240, 0.28760, 0.28760)
        rgb=(0.51570, 0.28430, 0.28430)
        rgb=(0.51901, 0.28099, 0.28099)
        rgb=(0.52231, 0.27769, 0.27769)
        rgb=(0.52562, 0.27438, 0.27438)
        rgb=(0.52893, 0.27107, 0.27107)
        rgb=(0.53223, 0.26777, 0.26777)
        rgb=(0.53554, 0.26446, 0.26446)
        rgb=(0.53884, 0.26116, 0.26116)
        rgb=(0.54215, 0.25785, 0.25785)
        rgb=(0.54545, 0.25455, 0.25455)
        rgb=(0.54876, 0.25124, 0.25124)
        rgb=(0.55207, 0.24793, 0.24793)
        rgb=(0.55537, 0.24463, 0.24463)
        rgb=(0.55868, 0.24132, 0.24132)
        rgb=(0.56198, 0.23802, 0.23802)
        rgb=(0.56529, 0.23471, 0.23471)
        rgb=(0.56860, 0.23140, 0.23140)
        rgb=(0.57190, 0.22810, 0.22810)
        rgb=(0.57521, 0.22479, 0.22479)
        rgb=(0.57851, 0.22149, 0.22149)
        rgb=(0.58182, 0.21818, 0.21818)
        rgb=(0.58512, 0.21488, 0.21488)
        rgb=(0.58843, 0.21157, 0.21157)
        rgb=(0.59174, 0.20826, 0.20826)
        rgb=(0.59504, 0.20496, 0.20496)
        rgb=(0.59835, 0.20165, 0.20165)
        rgb=(0.60165, 0.19835, 0.19835)
        rgb=(0.60496, 0.19504, 0.19504)
        rgb=(0.60826, 0.19174, 0.19174)
        rgb=(0.61157, 0.18843, 0.18843)
        rgb=(0.61488, 0.18512, 0.18512)
        rgb=(0.61818, 0.18182, 0.18182)
        rgb=(0.62149, 0.17851, 0.17851)
        rgb=(0.62479, 0.17521, 0.17521)
        rgb=(0.62810, 0.17190, 0.17190)
        rgb=(0.63140, 0.16860, 0.16860)
        rgb=(0.63471, 0.16529, 0.16529)
        rgb=(0.63802, 0.16198, 0.16198)
        rgb=(0.64132, 0.15868, 0.15868)
        rgb=(0.64463, 0.15537, 0.15537)
        rgb=(0.64793, 0.15207, 0.15207)
        rgb=(0.65124, 0.14876, 0.14876)
        rgb=(0.65455, 0.14545, 0.14545)
        rgb=(0.65785, 0.14215, 0.14215)
        rgb=(0.66116, 0.13884, 0.13884)
        rgb=(0.66446, 0.13554, 0.13554)
        rgb=(0.66777, 0.13223, 0.13223)
        rgb=(0.67107, 0.12893, 0.12893)
        rgb=(0.67438, 0.12562, 0.12562)
        rgb=(0.67769, 0.12231, 0.12231)
        rgb=(0.68099, 0.11901, 0.11901)
        rgb=(0.68430, 0.11570, 0.11570)
        rgb=(0.68760, 0.11240, 0.11240)
        rgb=(0.69091, 0.10909, 0.10909)
        rgb=(0.69421, 0.10579, 0.10579)
        rgb=(0.69752, 0.10248, 0.10248)
        rgb=(0.70083, 0.09917, 0.09917)
        rgb=(0.70413, 0.09587, 0.09587)
        rgb=(0.70744, 0.09256, 0.09256)
        rgb=(0.71074, 0.08926, 0.08926)
        rgb=(0.71405, 0.08595, 0.08595)
        rgb=(0.71736, 0.08264, 0.08264)
        rgb=(0.72066, 0.07934, 0.07934)
        rgb=(0.72397, 0.07603, 0.07603)
        rgb=(0.72727, 0.07273, 0.07273)
        rgb=(0.73058, 0.06942, 0.06942)
        rgb=(0.73388, 0.06612, 0.06612)
        rgb=(0.73719, 0.06281, 0.06281)
        rgb=(0.74050, 0.05950, 0.05950)
        rgb=(0.74380, 0.05620, 0.05620)
        rgb=(0.74711, 0.05289, 0.05289)
        rgb=(0.75041, 0.04959, 0.04959)
        rgb=(0.75372, 0.04628, 0.04628)
        rgb=(0.75702, 0.04298, 0.04298)
        rgb=(0.76033, 0.03967, 0.03967)
        rgb=(0.76364, 0.03636, 0.03636)
        rgb=(0.76694, 0.03306, 0.03306)
        rgb=(0.77025, 0.02975, 0.02975)
        rgb=(0.77355, 0.02645, 0.02645)
        rgb=(0.77686, 0.02314, 0.02314)
        rgb=(0.78017, 0.01983, 0.01983)
        rgb=(0.78347, 0.01653, 0.01653)
        rgb=(0.78678, 0.01322, 0.01322)
        rgb=(0.79008, 0.00992, 0.00992)
        rgb=(0.79339, 0.00661, 0.00661)
        rgb=(0.79669, 0.00331, 0.00331)
        rgb=(0.80000, 0.00000, 0.00000)
    }
}

